The Possibility of Fairness: Revisiting the Impossibility Theorem in Practice

The ``impossibility theorem'' -- which is considered foundational in algorithmic fairness literature -- asserts that there must be trade-offs between common notions of fairness and performance when fitting statistical models, except in two special cases: when the prevalence of the outcome being predicted is equal across groups, or when a perfectly accurate predictor is used. However, theory does not always translate to practice. In this work, we challenge the implications of the impossibility theorem in practical settings. First, we show analytically that, by slightly relaxing the impossibility theorem (to accommodate a \textit{practitioner's} perspective of fairness), it becomes possible to identify a large set of models that satisfy seemingly incompatible fairness constraints. Second, we demonstrate the existence of these models through extensive experiments on five real-world datasets. We conclude by offering tools and guidance for practitioners to understand when -- and to what degree -- fairness along multiple criteria can be achieved. For example, if one allows only a small margin-of-error between metrics, there exists a large set of models simultaneously satisfying \emph{False Negative Rate Parity}, \emph{False Positive Rate Parity}, and \emph{Positive Predictive Value Parity}, even when there is a moderate prevalence difference between groups. This work has an important implication for the community: achieving fairness along multiple metrics for multiple groups (and their intersections) is much more possible than was previously believed.

==> authors.tex <==
\author{Andrew Bell}
\affiliation{%
  \institution{New York University}
  \streetaddress{50 West 4th St}
  \city{New York}
  \country{United States}}
\email{alb9742@nyu.edu}

\author{Lucius Bynum}
\affiliation{%
  \institution{New York University}
  \streetaddress{50 West 4th St}
  \city{New York}
  \country{United States}}
\email{lucius@nyu.edu}

\author{Nazarii Drushchak}
\affiliation{%
  \institution{Ukrainian Catholic University}
% \streetaddress{50 West 4th St}
  \city{Lviv}
  \country{Ukraine}}
\email{naz2001r@gmail.com}

\author{Tetiana Herasymova}
\affiliation{%
  \institution{Ukrainian Catholic University}
% \streetaddress{50 West 4th St}
  \city{Lviv}
  \country{Ukraine}}
\email{t.herasymova@ucu.edu.ua}

\author{Lucas Rosenblatt}
\affiliation{%
  \institution{New York University}
  \streetaddress{50 West 4th St}
  \city{New York}
  \country{United States}}
\email{lucas.rosenblatt@nyu.edu}

\author{Julia Stoyanovich}
\affiliation{%
  \institution{New York University}
  \streetaddress{50 West 4th St}
  \city{New York}
  \country{United States}}
\email{stoyanovich@nyu.edu}

==> deprecated.tex <==
\begin{equation*}
\begin{array}{llll}
\text{maximize}  & \displaystyle\sum\limits_{i=1}^{n}  x_{i} \cdot l_{i}                                                                   &                 & \\
\text{subject to}& \displaystyle\sum\limits_{i=1}^{n}  x_{i} = k,                                                                          &                 & \text{(KLS)}\\
                 & \displaystyle\sum\limits_{i=1}^{n}  x_{i} \cdot g_{j_i} \leq 1.2 \displaystyle\sum\limits_{i=1}^{n} x_{i} \cdot g_{ref_i},  & \forall j \in G, j \ne ref & \text{(ESU)}\\
                 & \displaystyle\sum\limits_{i=1}^{n}  x_{i} \cdot g_{j_i} \geq 0.8 \displaystyle\sum\limits_{i=1}^{n} x_{i} \cdot g_{ref_i},  & \forall j \in G, j \ne ref & \text{(ESL)}\\
                 & \frac{1}{P_{g_{j_i}}}\displaystyle\sum\limits_{i=1}^{n}  x_{i} \cdot g_{j_i} \leq \frac{1.2}{P_{g_{ref_i}}} \displaystyle\sum\limits_{i=1}^{n} x_{i} \cdot g_{ref_i},    &\forall j \in G, j \ne ref & \text{(RU)}\\
                 & \frac{1}{P_{g_{j}}}\displaystyle\sum\limits_{i=1}^{n}  x_{i} \cdot g_{j_i} \geq \frac{0.8}{P_{g_{ref}}} \displaystyle\sum\limits_{i=1}^{n} x_{i} \cdot g_{ref_i},    &\forall j \in G, j \ne ref & \text{(RL)}\\
                 &                                                & x_{i}, l_{i} \in \{0,1\}, &i=1 ,\dots, n & \\
                 &                                                & g_{j_i} \in \{0,1\}, & j \in G & \\
                 &                                                & P_{g_j}} = \displaystyle\sum\limits_{i=1}^{n} g_{j_i} \cdot l_{i} & j \in G & \\
\end{array}
\end{equation*}

Where $N$ is the set of entities, $n = |N|$, $x$ is a binary array of length $n$ where entry $x_i$ indicates whether or not entity $i \in N$ is included in the final list, $l$ is a binary array of length $n$ such that $l_{i} = 1$ if the outcome entity $x_i, i \in N$ is 1 and 0 otherwise, $G$ is a set of protected groups, $g_{j}$ is a binary array of length $n$ where entry $g_{j}_{i}$ indicates whether or not entry entity $i \in N$ is in group $j$, and $k$ is the final list size. Note that group $g_{ref}$ is the reference group for disparity calculations. KLS is the ``k-list-size'' constraint, ESU and ESL are the upper and lower bounds for the equal selection constraint respectively, and RU and RL are the upper and lower bounds for the recall parity constraint respectively.

\section{Constraint Program Details}\label{sec:constraint_program}

\begin{figure}
\centering
\subfloat[$|\epsilon_\alpha|, |\epsilon_\beta|, |\epsilon_v| \leq 0.02 \\ \sum\limits_{p_1,p_2} a_{p_1,p_2} = 134484$]
{\includegraphics[width=.3\textwidth]{figures/e=0.02_sum=134484.0.png}}
\subfloat[$|\epsilon_\alpha|, |\epsilon_\beta|, |\epsilon_v| \leq 0.05 \\ \sum\limits_{p_1,p_2} a_{p_1,p_2} = 331244$]
{\includegraphics[width=.3\textwidth]{figures/e=0.05_sum=331244.0.png}
}
\subfloat[$|\epsilon_\alpha|, |\epsilon_\beta|, |\epsilon_v| \leq 0.1 \\ \sum\limits_{p_1,p_2} a_{p_1,p_2} = 861052$]
{\includegraphics[width=.3\textwidth]{figures/e=0.1_sum=861052.0.png}
}
\caption{Effect of varying group prevalence $p_1, p_2$ on number of CP solutions, where $PPV \in \lbrack 0, 1.0 \rbrack $}
\label{fig:cp_solutions}
\end{figure}

A constraint program (CP) provides an alternative means of measuring how large the space of feasible solutions is for a given setting of tolerances, such as $|\epsilon_\alpha|, |\epsilon_\beta|, |\epsilon_v| \leq 0.05$. Rather than estimate the area taken up on a discretized plot of two dimensions --- $PPV_2$ and $FNR_2$ --- we can consider all dimensions simultaneously, simply as a set of \emph{feasible solutions} to a constraint program. Using the CP-SAT solver in Google ORTools, we express our problem's governing equations as a set of integer variables and constraints. Our quantities of interest ($FPR, FNR, PPV, p, \epsilon_\alpha, \epsilon_\beta, \epsilon_v, \epsilon_p$) are all real numbers rather than integers, with infinitely many possible values in their respective ranges. To characterize the size of the solution space for different tolerances, we discretize the interval $[0, 1]$ into $N + 1$ bins (and correspondingly, the interval $[-1, 1]$ into $2N + 1$ bins). For example, an $FPR$ value of 0.9 would correspond to an integer value of 9 when $N=10$. With this discretization, we represent our problem using the following constraint program:

\begin{equation*}
\begin{array}{rll}
    \alpha_i, \beta_i, p_i, v_i &\in [0, N] \ \text{integer} & \forall i \in \{1, 2\}\\
    \epsilon_j &\in [-N, N] \ \text{integer} & \forall j \in \{\alpha, \beta, p, v\}\\
    m_i, d_i &\in [0, N^2] \ \text{integer} & \forall i \in \{1, 2\}\\
    n_i &\in [0, N^3] \ \text{integer} & \forall i \in \{1, 2\}\\\\
    
    p_i &= b_i \cdot N & \forall i \in \{1, 2\}\\

    j_1 &= j_2 + \epsilon_{j} & \forall j \in \{\alpha, \beta, p, v\}\\\\

    \epsilon_{j} &\geq -\epsilon_{\text{max}} \cdot N & \forall j \in \{\alpha, \beta, v\}\\
    \epsilon_{j} &\leq \epsilon_{\text{max}} \cdot N & \forall j \in \{\alpha, \beta, v\}\\\\

    m_i &= p_i \cdot (N - v_i) & \forall i \in \{1, 2\}\\
    n_i &= m_i \cdot (N - \beta_i) & \forall i \in \{1, 2\}\\
    d_i &= v_i \cdot (N - p_i) & \forall i \in \{1, 2\}\\
    n_i &= \alpha_i \cdot d_i & \forall i \in \{1, 2\}\\

    
\end{array}
\end{equation*}

where $N$ is the number of integers; $n, m, d$ are intermediate variables used to represent multiplicative constraints for the CP-SAT solver; $\epsilon_{\text{max}}$ represents the maximum allowable value of $|\epsilon_\alpha|, |\epsilon_\beta|, |\epsilon_v|$; $b_i$ represent the observed base rates in the real-valued range $[0, 1]$; and as in the main body of the paper, $\alpha, \beta, v$ represent $FPR, FNR, PPV$. The CP-SAT solver allows us to enumerate all possible solutions to a constraint program. With $N^6$ possible values for the set $\{FPR_1, FPR_2, FNR_1, FNR_2, PPV_1, PPV_2\}$, for any fixed $N$, we can characterize the size of the discretized solution space as a function of changes to the other inputs simply as the number of feasible solutions --- analogous to a discretized fairness `volume' instead of the fairness area in Section~\ref{sec:theory}. Figure~\ref{fig:cp_solutions} and Figure~\ref{fig:cp_varying_ppv} show plots of the number of feasible CP solutions with $N=100$ corresponding to the same parameter settings used in Figure~\ref{fig:varying_e_p} and Figure~\ref{fig:varying_ppv}.

\begin{figure}
\centering
\subfloat[$PPV \in \lbrack0,0.33\rbrack \\ \sum\limits_{p_1,p_2} a_{p_1,p_2} = 59084$]
{\includegraphics[width=.3\textwidth]{figures/e=0.05, PPV in [(0.0, 0.33)]_sum=59084.0.png}}
\subfloat[$PPV \in \lbrack0.33,0.67\rbrack \\ \sum\limits_{p_1,p_2} a_{p_1,p_2} = 57857$]
{\includegraphics[width=.3\textwidth]{figures/e=0.05, PPV in [(0.33, 0.67)]_sum=57857.0.png}
}
\subfloat[$PPV \in \lbrack0.67,1.0\rbrack \\ \sum\limits_{p_1,p_2} a_{p_1,p_2} = 208827$]
{\includegraphics[width=.3\textwidth]{figures/e=0.05, PPV in [(0.67, 1.0)]_sum=208827.0.png}
}
\caption{Effect of varying $PPV$ on number of CP solutions, where $|\epsilon_\alpha|, |\epsilon_\beta|, |\epsilon_v| \leq 0.05$}
\label{fig:cp_varying_ppv}
\end{figure}

==> loose_ends.tex <==
[ ] Review and format appendix
[ ] Add analysis for number of grid points
[ ] Add sample sizes below table

==> outline.tex <==
% i) intro
% ii) related work
% iii) relaxation constraints and showing what will happen
% iv) fair set selection
% v) empirical results demonstrating the fairness evaluator
% iv) discussion and conclusion

==> proofs.tex <==
\section{Proofs}
\label{sec:proofs}

Consider the following, which follow directly from Chouldechova~\cite{chouldechova2016fair}:

\begin{align}
    \text{FPR}_{g_1} &= \frac{p_{g_1}}{1 - p_{g_1}} \frac{1-\text{PPV}_{g_1}}{\text{PPV}_{g_1}}(1-\text{FNR}_{g_1}) \\
    \text{FPR}_{g_2} &= \frac{p_{g_2}}{1 - p_{g_2}} \frac{1-\text{PPV}_{g_2}}{\text{PPV}_{g_2}}(1-\text{FNR}_{g_2})
\end{align}

Suppose that $\text{PPV}_{g_1} = \text{PPV}_{g_2}$ and that $\text{FNR}_{g_1} = \text{FNR}_{g_2}$. We can then express the FPR disparity with respect to $g_2$ in the following way:

\begin{align}
    \frac{\text{FPR}_{g_1}}{\text{FPR}_{g_2}} &= \frac{p_{g_1} ( 1 - p_{g_2})}{p_{g_2} ( 1- p_{g_1})}
\end{align}

Using this expression for the FPR disparity in terms of group prevelances, we can create the following plot in which the highlighted region shows all the pairs of prevalences $(p_{g_1}, p_{g_2}})$ for which  $0.8 \leq \frac{\text{FPR}_{g_1}}{\text{FPR}_{g_2}} \leq 1.2$ is true:

\begin{figure}[h!]
    \centering
    \includegraphics[width=4.0cm]{figures/prev_region.png}
    %\caption{Visualizations of the filters $W_1$, $W_2$, respectively.}
    %\label{fig:survey_flow}
\end{figure}

The implication 







==> tables/fairness_metrics.tex <==
\begin{center}
\begin{table}
\caption{\andrew{Table that may or may not make it into the paper}}
\begin{tabular}{ |c|c| } 
    \hline
    Metric & heading2 \\
    \hline
    Equal selection, demographic parity, statistical parity & - \\
    Disparate impact, proportional parity & - \\ 
    Equalized odds & - \\
    Equal opportunity & - \\
    False positive parity & - \\ 
    False negative parity & - \\
    False discovery parity & - \\
    False omission parity & - \\
    Recall, hit rate, true positive rate & - \\
    Precision, positive predictive value & - \\
    Equal opportunity difference & - \\
    Average odds difference & - \\
    Theil index & - \\
    Distance b/w privileged and unprivileged (ex. Euclidean, Mahalanobis) & - \\
    Bounded group loss & - \\
    Accuracy metric parity & - \\

    \hline
\end{tabular}
\label{table:fairness_metrics}
\end{table}
\end{center}

==> tables/guidance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{When can one expect a high number of feasible models that satisfy fairness constraints for \\ \fpr, \fnr, and \ppv within a 5\% margin?}
\label{tab:guidance}
\centering
\begin{tabular}{p{7cm}|p{7cm}}
\textbf{Factors \emph{increasing} the number of feasible models} & \textbf{Factors \emph{decreasing} the number of feasible models} \\ \hline
\textbullet~Overall prevelance is close to 50\% & \textbullet~Overall prevelance is close to 0\% or 100\% \\
\textbullet~Maximum pairwise prevelance difference between groups is less than 10\% & \textbullet~Maximum pairiwse prevelance difference between groups is greater than 20\% \\
\textbullet~PPV of the classifier is greater than or equal to 67\% & \textbullet~PPV of the classifier is less than 67\%
\end{tabular}
\end{table}


